Gameplay Filters: Robust Zero-Shot Safety through Adversarial Imagination

Despite the impressive recent advances in learning-based robot control, ensuring robustness to out-of-distribution conditions remains an open challenge. Safety filters can, in principle, keep arbitrary control policies from incurring catastrophic failures by overriding unsafe actions, but existing solutions for complex (e.g., legged) robot dynamics do not span the full motion envelope and instead rely on local, reduced-order models. These filters tend to overly restrict agility and can still fail when perturbed away from nominal conditions. This paper presents the gameplay filter, a new class of predictive safety filter that continually plays out hypothetical matches between its simulation-trained safety strategy and a virtual adversary co-trained to invoke worst-case events and sim-to-real error, and precludes actions that would cause failures down the line. We demonstrate the scalability and robustness of the approach with a first-of-its-kind full-order safety filter for (36-D) quadrupedal dynamics. Physical experiments on two different quadruped platforms demonstrate the superior zero-shot effectiveness of the gameplay filter under large perturbations such as tugging and unmodeled terrain. Experiment videos and open-source software are available online: https://saferobotics.org/research/gameplay-filter

==> l_step_gameplay_filter.tex <==
\newcommand{\result}{{\text{res}}}

\begin{algorithm}[!t]
\caption{Real-Time Gameplay Safety Filter}
\label{alg:gp_monitor}
\begin{algorithmic}[1]
    % \color{teal}
    \Require $\xcur, \policyTask, \fallback, \actorDstb, \dyn, \phorizon, \khorizon$
        \State $\xplan{0} \gets \xcur$
        \For{$\tplan=0$ to $\khorizon$}
            \If{$\tplan = 0$}
                \State $\policyCtrl \gets \policyTask$\Comment{Evaluate the task policy}
            \Else
                \State $\policyCtrl \gets \fallback$\Comment{Followed by the fallback}
            \EndIf
            \State $\cplancur \gets \policyCtrl(\xplancur)$
            % \State $\dplancur \gets \actorDstb(\xplancur, \cplancur)$
            \State $\dplancur \gets \actorDstb(\xplancur)$
            \State $\xplannxt \gets \dyn(\xplancur,\cplancur,\dplancur)$
            \If{$\consFunc(\xplannxt) < 0$}\Comment{Gameplay violates safety}
                \State $\result \gets 0$
                \State \Return $\result, \fallback$
            \EndIf
            \If{$\targFunc(\xplannxt) > 0$}\Comment{Gameplay succeeds}
                \State $\result \gets 1$
                \State \Return $\result, \policyTask$
            \EndIf
        \EndFor
        $\result \gets 0$\Comment{Gameplay does not reach}
        \State \Return $\result, \fallback$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[!t]
\caption{$\phorizon$-Step Gameplay Safety Filter}
\label{alg:ell_gp_monitor}
\begin{algorithmic}[1]
    % \Function{Gameplay with latency}{$\xcur, \policyTask, \result_{\tdisc-1}, L, \khorizon$}
    % \Require $\xcur, \result_{\tdisc-1}, \policyTask, \fallback, \actorDstb, \dyn, \phorizon, \khorizon$
    \Require $\xcur, \policyTask, \policyExec, \fallback, \actorDstb, \dyn, \phorizon, \khorizon$
        \State $\xplan{0} \gets \xcur$
        % \State $\cplan{0}, \ccur \gets \policyTask(\xcur)$
        % \If{$\result_{\tdisc-1}$}\Comment{Previous gameplay succeeded}
        %     \State $\policyExec \gets \policyTask$\Comment{Use (verified) task policy}
        % \Else
        %     \State $\policyExec \gets \fallback$
        % \EndIf
        % \For{\remove{$\tplan=0$ \text{to} $\phorizon$}}
        %     \State \remove{$\cplancur \gets \policyExec(\xplancur)$}
        %     % \State \remove{$\dplancur \gets \actorDstb(\xplancur, \cplancur)$}
        %     \State \remove{$\dplancur \gets \actorDstb(\xplancur)$}
        %     \State \remove{$\xplancur \gets \dyn(\xplancur,\cplancur,\dplancur)$}
        % \EndFor
        \For{$\tplan=0$ to $\khorizon$}
            \If{\new{$\tplan < \phorizon$}}
                \State \new{$\policyCtrl \gets \policyExec$}  \Comment{Apply the verified filter}
            \ElsIf{$\tplan < 2\phorizon$}
                \State $\policyCtrl \gets \policyTask$  \Comment{Evaluate the task policy}
            \Else
                \State $\policyCtrl \gets \fallback$  \Comment{Followed by the fallback}
            \EndIf
            \State $\cplancur \gets \policyCtrl(\xplancur)$
            % \State $\dplancur \gets \actorDstb(\xplancur, \cplancur)$
            \State $\dplancur \gets \actorDstb(\xplancur)$
            \State $\xplannxt \gets \dyn(\xplancur,\cplancur,\dplancur)$
            \If{$\consFunc(\xplannxt) < 0$}  \Comment{Gameplay violates safety}
                \State $\result \gets 0$
                \State \Return $\result, \fallback$
            \EndIf
            \If{$\targFunc(\xplannxt) > 0$ and $\tplan\geq2\phorizon$}  \Comment{Gameplay succeeds}
                \State $\result \gets 1$
                \State \Return $\result, \policyTask$
            \EndIf
        \EndFor
        $\result \gets 0$  \Comment{Gameplay does not reach}
        \State \Return $\result, \fallback$
    % \EndFunction
\end{algorithmic}
\end{algorithm}

==> misc.tex <==
\begin{table*}[!ht]
    \centering
    \begin{tabular}{|c|c|c|ccc|}
    \hline
    \multirow{2}{*}{Policy} & \multirow{2}{*}{Cost} & \multirow{2}{*}{Safety filter} & \multicolumn{3}{c|}{Metric} \\ 
    \cline{4-6} & & & \multicolumn{1}{c|}{Safe rate} & \multicolumn{1}{c|}{Shield rate} & Distance \\ 
    \hline
    \multirow{3}{*}{ISAACS} & \multirow{3}{*}{RA margin} & Value-based & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \\
    \cline{3-6} & & Naive rollout & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \\ 
    \cline{3-6} & & Gameplay & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \\ 
    \hline
    \multirow{3}{*}{ISAACS} & \multirow{3}{*}{RA penalty} & Value-based & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \\
    \cline{3-6} & & Naive rollout & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \\ 
    \cline{3-6} & & Gameplay & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \\ 
    \hline
    \multirow{3}{*}{\makecell{Naive SAC \\ (no disturbance)}} & \multirow{3}{*}{RA margin} & Value-based & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \\
    \cline{3-6} & & Naive rollout & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \\ 
    \cline{3-6} & & Gameplay & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \\ 
    \hline
    \multirow{3}{*}{\makecell{Naive SAC \\ (no disturbance)}} & \multirow{3}{*}{RA penalty} & Value-based & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \\
    \cline{3-6} & & Naive rollout & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \\ 
    \cline{3-6} & & Gameplay & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \\ 
    \hline
    Task policy & n/a & n/a & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} \\
    \hline
    \end{tabular}
    \caption{Simulated result comparison between different policies, costs, safety filters, 50 different runs}
    \label{tab:my_label}
\end{table*}

\todo{better figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[clip, trim=0.5cm 1.0cm 53cm 1.0cm, height=45pt]{figures/train-avoid-eval-reachavoid.pdf}
    \includegraphics[clip, trim=72.5cm 1.0cm 0.0cm 1.0cm, height=45pt]{figures/train-avoid-eval-reachavoid.pdf}
    \caption{Train avoid, eval reachavoid}
    \label{fig:avoid-ra}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[clip, trim=0.5cm 1.0cm 53cm 1.0cm, height=45pt]{figures/train-reachavoid-eval-failure.pdf}
    \includegraphics[clip, trim=72.5cm 1.0cm 0.0cm 1.0cm, height=45pt]{figures/train-reachavoid-eval-failure.pdf}
    \caption{Train reachavoid, eval failure}
    \label{fig:ra-avoid}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[clip, trim=0.5cm 1.0cm 53cm 1.0cm, height=45pt]{figures/train-reachavoid-eval-reachavoid.pdf}
    \includegraphics[clip, trim=72.5cm 1.0cm 0.0cm 1.0cm, height=45pt]{figures/train-reachavoid-eval-reachavoid.pdf}
    \caption{Train reachavoid, eval reachavoid}
    \label{fig:ra-ra}
\end{figure}

==> naive_gameplay_filter.tex <==
\begin{algorithm}
\caption{Gameplay Safety Filter}
\label{alg:gameplay}
\begin{algorithmic}[1]
    % \Function{Gameplay}{$\xcur, \policyTask, \khorizon$}
    \Require $\xcur, \policyTask, \khorizon$
        \State $\xplan{0} \gets \xcur$
        \State $\cplan{0}, \ccur \gets \policyTask(\xcur)$
        \State $\dplan{0} \gets \policyDstb(\xplan{0}, \cplan{0})$
        \State $\xplan{1}\gets \dyn(\xplan{0},\cplan{0},\dplan{0})$
        \If{$\consFunc(\xplan{1}) < 0$}
            \State \Return $\fallback(\xcur)$\Comment{Gameplay is failed}
        \EndIf
        \For{$\tplan=1$ \text{to} $\khorizon$}
            \State $\cplancur \gets \fallback(\xplancur)$
            \State $\dplancur \gets \policyDstb(\xplancur, \cplancur)$
            \State $\xplancur \gets \dyn(\xplancur,\cplancur,\dplancur)$
            \If{$\consFunc(\xplancur) < 0$}
                \State \Return $\fallback(\xcur)$\Comment{Gameplay is failed}
            \EndIf
            \If{$\targFunc(\xplancur) > 0$}
                \State \Return $\ccur$\Comment{Gameplay is successful}
            \EndIf
        \EndFor
        \State \Return $\fallback(\xcur)$\Comment{Gameplay is failed}
    % \EndFunction
\end{algorithmic}
\end{algorithm}

==> notation_rebuttal.tex <==
% This file contains the notation macros for the entire paper.
\usepackage{fontawesome5}  % Icons

% ---------------- Notation ----------------
% Operators
\newcommand{\wt}{{\widetilde}}
\newcommand{\wh}{{\widehat}}
\newcommand{\ol}{{\overline}}
\newcommand{\ul}{{\underline}}
\newcommand{\lra}{{\Longleftrightarrow}}
\newcommand{\ra}{{\rightarrow}}
\DeclareMathOperator*{\st}{{\mathop{\text{s.t.}}}}
\renewcommand{\ae}{{\mathop{\text{a.e.}}}}
\DeclareMathOperator*{\argmax}{{\mathop{\mathrm{argmax}}}}
\DeclareMathOperator*{\argmin}{{\mathop{\mathrm{argmin}}}}
\newcommand{\falsum}{{\Rightarrow\!\Leftarrow}}
\DeclareMathOperator*{\expect}{{\mathbb{E}}}
\DeclareMathOperator{\interior}{{int}}
\DeclareMathOperator{\sgn}{{sgn}}
\DeclareMathOperator{\cov}{{\mathrm{Cov}}}
\DeclareMathOperator*{\var}{{\mathrm{Var}}}
\newcommand{\sgnDist}[1]{{s_{#1}}}
\newcommand{\indicator}{\mathbbm{1}}
\renewcommand{\inf}{\mathop{\mathrm{inf}\vphantom{\mathrm{sup}}}}  % same height
\newcommand{\loss}{{L}}
\newcommand{\iter}{{i}}

% Sets and spaces
\newcommand{\reals}{\mathbb{R}}
\newcommand{\naturals}{\mathbb{N}}
\newcommand{\rationals}{\mathbb{Q}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\compl}{\text{c}}  % {\mathsf{c}}
\renewcommand{\complement}{\text{c}}  % {\mathsf{c}}
\newcommand{\boundary}{{\partial}}
\newcommand{\ball}{{B}}
\newcommand{\radius}{{r}}
\newcommand{\simplex}[1]{{\Delta#1}}
\newcommand{\ones}{{\mathbf{1}}}
\renewcommand{\emptyset}{{\text{\O}}}  % a prettier empty set symbol
% \renewcommand{\emptyset}{{\varnothing}} 

% Probability
% \newcommand{\prob}{\text{Pr}}
\newcommand{\prob}{{P}}
\newcommand{\probDens}{{p}}
\newcommand{\gaussian}{{\mathcal{N}}}
\newcommand{\gp}{{\mathcal{GP}}}
\newcommand{\kl}{{D_{KL}}}
\newcommand{\mi}{\text{MI}}
\newcommand{\crossentropy}{\text{CE}}
\newcommand{\entropy}{{\mathcal{H}}}
\newcommand{\probd}{{\probDens_\dSet}}
\newcommand{\probx}{{\probDens_\state}}
\newcommand{\probtraj}{{\probDens_\traj}}
\newcommand{\covK}{{\mathbf{K}}}

\newcommand{\dataAll}{{\mathbf{X}}}
\newcommand{\dataVec}{{\mathbf{x}}}
\newcommand{\hiddenVec}{{\boldsymbol{\theta}}}
\newcommand{\priorParamVec}{{\boldsymbol{\alpha}}}
\newcommand{\data}{{x}}
\newcommand{\hidden}{{\theta}}
\newcommand{\priorParam}{{\alpha}}
\newcommand{\iid}{\mathrel{\overset{\makebox[0pt]{\mbox{\tiny i.i.d.}}}{\sim}}}
\newcommand{\CVaR}{{\text{CVaR}}}
\newcommand{\VaR}{{\text{VaR}}}


% exponential family
\newcommand{\natParam}{{\eta}}
\newcommand{\suffStats}{{T}}
\newcommand{\logPart}{{A}}
\newcommand{\baseMeas}{{h}}


% Calculus
\newcommand{\grad}{{\nabla}}
\newcommand{\gradx}{{\nabla_\state}}
\newcommand{\totalDeriv}{{D}}


% NN
\newcommand{\batch}{{\mathcal{B}}}
\newcommand{\clf}{{h}}


% Dynamical system
\newcommand{\state}{{x}}
\newcommand{\statecont}{{\state_c}}
\newcommand{\statedisc}{{\state_d}}
\newcommand{\stateaux}{{\tilde{\state}}}
\newcommand{\statenxt}{{\state'}}
% \newcommand{\stateimag}[2]{{\state_{#1|#2}}}
\newcommand{\ctrl}{{u}}
\newcommand{\ctrlaux}{{\tilde{\ctrl}}}
% \newcommand{\ctrlimag}[2]{{\ctrl_{#1|#2}}}
\newcommand{\ctrlnxt}{{\ctrl'}}
\newcommand{\dstb}{{d}}
\newcommand{\dstbaux}{{\tilde{\dstb}}}
% \newcommand{\dstbimag}[2]{{\dstb_{#1|#2}}}
\newcommand{\dstbnxt}{{\dstb'}}
\newcommand{\obsrv}{{y}}
\newcommand{\info}{{\eta}}
\newcommand{\belief}{{b}}
\newcommand{\dstbmax}{{d_{\max}}}


% \newcommand{\xplan}[2]{{\hat \state}_{#1 \mid #2}}
% \newcommand{\cplan}[2]{{\hat \ctrl}_{#1 \mid #2}}
\newcommand{\xplan}[1]{{\hat \state}_{#1}}
\newcommand{\cplan}[1]{{\hat \ctrl}_{#1}}
\newcommand{\dplan}[1]{{\hat \dstb}_{#1}}
\newcommand{\xplancur}{\xplan{\tplan}}
\newcommand{\cplancur}{\cplan{\tplan}}
\newcommand{\dplancur}{\dplan{\tplan}}
\newcommand{\xplannxt}{\xplan{\tdisc+1}}
\newcommand{\cplannxt}{\cplan{\tdisc+1}}
% \newcommand{\error}[2]{{e}_{#1 \mid #2}}
\newcommand{\error}[1]{e_{#1}}
\newcommand{\errorcur}{\error{\tdisc}}
\newcommand{\errornxt}{\error{\tdisc+1}}
\newcommand{\tplan}{{\tau}}
\newcommand{\tplanaux}{{s}}
\newcommand{\traj}{{\mathbf{\state}}}
% \newcommand{\traj}{{\xi}}
% \newcommand{\trajplan}{{\mathbf{z}}}
% \newcommand{\csigplan}{{\mathbf{v}}}
\newcommand{\trajplan}{{\hat \traj}}
\newcommand{\csigplan}{{\hat \csig}}
\newcommand{\csig}{{\mathbf{\ctrl}}}
\newcommand{\csigaux}{{\tilde{\csig}}}
\newcommand{\dsig}{{\mathbf{\dstb}}}
\newcommand{\obsrvtraj}{{\mathbf{\obsrv}}}
\newcommand{\xSet}{{\mathcal{X}}}
% \newcommand{\xSet}{{\mathcal{S}}}
\newcommand{\cSet}{{\mathcal{U}}}
\newcommand{\dSet}{{\mathcal{D}}}
% \newcommand{\xSet}{{\reals^\nx}}
% \newcommand{\cSet}{{\reals^\nc}}
% \newcommand{\dSet}{{\reals^\nd}}
% \newcommand{\xplanSet}{{\mathcal{Z}}}
% \newcommand{\cplanSet}{{\mathcal{V}}}
\newcommand{\xplanSet}{{\hat\xSet}}
\newcommand{\cplanSet}{{\hat\cSet}}
\newcommand{\infoSet}{{\mathcal{H}}}
%\newcommand{\trajSet}{{\mathbb{X}}}
% \newcommand{\trajSet}{{\mathbb{S}}}
\newcommand{\trajSet}{{\Xi}}
\newcommand{\csigSet}{{\mathbb{U}}}
\newcommand{\dsigSet}{{\mathbb{D}}}
\newcommand{\trajParam}{{\theta}}
\newcommand{\trajParamSet}{{\Theta}}


\newcommand{\nx}{{n_\state}}
\newcommand{\nc}{{n_\ctrl}}
\newcommand{\nd}{{n_\dstb}}
\newcommand{\nci}{{n_{\ctrl_\iagent}}}
\newcommand{\naux}{{m}}

\newcommand{\dyn}{{f}} % dynamics
\newcommand{\dyninfo}{\dyn^\info}
\newcommand{\dynNom}{{\bar{\dyn}}}
\newcommand{\dynCont}{\dyn^c}
\newcommand{\dynContNom}{{\bar{\dynCont}}}
\newcommand{\dynSet}{\reach}
% \newcommand{\dynContSet}{\mathcal{F}}
\newcommand{\dynContSet}{\reach^c}
\newcommand{\dynTrue}{{\dyn^*}}
\newcommand{\dynParam}{{\theta}}
\newcommand{\dynParamSet}{{\Theta}}
\newcommand{\sense}{{h}}  % measurement
% \newcommand{\deltat}{{\Delta \tcont}}
\newcommand{\deltat}{{\delta}}

\newcommand{\tcont}{{t}} % continuous time step
\newcommand{\tcontaux}{{\tau}}
\newcommand{\tcontauxaux}{{s}}
% \newcommand{\tinit}{{\tcont_0}}
\newcommand{\tinit}{0}
\newcommand{\tend}{\khorizon}

\newcommand{\tdisc}{{k}} % discrete time step
\newcommand{\tdiscaux}{{\tau}}
\newcommand{\tdiscauxaux}{{s}}
\newcommand{\tdiscstart}{{\tdisc_0}}
\newcommand{\khorizon}{{H}}
\newcommand{\phorizon}{{L}}

\newcommand{\xcur}{{\state_\tdisc}}
\newcommand{\ccur}{{\ctrl_\tdisc}}
\newcommand{\dcur}{{\dstb_\tdisc}}
\newcommand{\xnxt}{{\state_{\tdisc+1}}}
\newcommand{\cnxt}{{\ctrl_{\tdisc+1}}}
\newcommand{\dnxt}{{\dstb_{\tdisc+1}}}
\newcommand{\xterm}{{\state_\khorizon}}
\newcommand{\cterm}{{\ctrl_\khorizon}}
\newcommand{\dterm}{{\dstb_\khorizon}}
\newcommand{\xinit}{{\state_0}}
\newcommand{\cinit}{{\ctrl_0}}
\newcommand{\dinit}{{\dstb_0}}

\newcommand{\fx}[1]{{\dyn_{\state, #1}}}
\newcommand{\fu}[1]{{\dyn_{\ctrl, #1}}}
\newcommand{\fd}[1]{{\dyn_{\dstb, #1}}}
\newcommand{\rx}[1]{{\reward_{\state, #1}}}
\newcommand{\ru}[1]{{\reward_{\ctrl, #1}}}
\newcommand{\fxx}[1]{{\dyn_{\state\state, #1}}}
\newcommand{\fuu}[1]{{\dyn_{\ctrl\ctrl, #1}}}
\newcommand{\fux}[1]{{\dyn_{\ctrl\state, #1}}}
\newcommand{\rxx}[1]{{\reward_{\state\state, #1}}}
\newcommand{\ruu}[1]{{\reward_{\ctrl\ctrl, #1}}}
\newcommand{\rux}[1]{{\reward_{\ctrl\state, #1}}}
\newcommand{\fxcur}{\fx{\tdisc}}
\newcommand{\fucur}{\fu{\tdisc}}
\newcommand{\fdcur}{\fd{\tdisc}}
\newcommand{\fxxcur}{\fxx{\tdisc}}
\newcommand{\fuucur}{\fuu{\tdisc}}
\newcommand{\fuxcur}{\fux{\tdisc}}
\newcommand{\rxcur}{\rx{\tdisc}}
\newcommand{\rucur}{\ru{\tdisc}}
\newcommand{\rxxcur}{\rxx{\tdisc}}
\newcommand{\ruucur}{\ruu{\tdisc}}
\newcommand{\ruxcur}{\rux{\tdisc}}

\newcommand{\vx}[1]{{\valFunc_{\state, #1}}}
\newcommand{\qx}[1]{{\qFunc_{\state, #1}}}
\newcommand{\qu}[1]{{\qFunc_{\ctrl, #1}}}
\newcommand{\vxx}[1]{{\valFunc_{\state\state, #1}}}
\newcommand{\qxx}[1]{{\qFunc_{\state\state, #1}}}
\newcommand{\quu}[1]{{\qFunc_{\ctrl\ctrl, #1}}}
\newcommand{\qux}[1]{{\qFunc_{\ctrl\state, #1}}}
\newcommand{\vxcur}{\vx{\tdisc}}
\newcommand{\qxcur}{\qx{\tdisc}}
\newcommand{\qucur}{\qu{\tdisc}}
\newcommand{\vxxcur}{\vxx{\tdisc}}
\newcommand{\qxxcur}{\qxx{\tdisc}}
\newcommand{\quucur}{\quu{\tdisc}}
\newcommand{\quxcur}{\qux{\tdisc}}
\newcommand{\psdcoeff}{{\alpha}}

\newcommand{\deltax}{\delta\state}
\newcommand{\deltac}{\delta\ctrl}
\newcommand{\deltad}{\delta\dstb}
\newcommand{\deltaq}{\delta\qFunc}
\newcommand{\deltav}{\delta\valFunc}
\newcommand{\deltaxcur}{{\deltax_\tdisc}}
\newcommand{\deltaccur}{{\deltac_\tdisc}}
\newcommand{\deltadcur}{{\deltad_\tdisc}}
\newcommand{\deltaqcur}{{\deltaq_\tdisc}}
\newcommand{\deltavcur}{{\deltav_\tdisc}}

\newcommand{\lqcl}[1]{{K_{#1}}}
\newcommand{\lqol}[1]{{\kappa_{#1}}}
\newcommand{\lqclcur}{\lqcl{\tdisc}}
\newcommand{\lqolcur}{\lqol{\tdisc}}

% Optimal control and dynamic games
\newcommand{\outcome}{{J}}  % {{\mathcal{V}}}
\newcommand{\outcomeTask}{{\outcome^\task}}
\newcommand{\valFunc}{{V}}
\newcommand{\qFunc}{{Q}}

\newcommand{\policy}{{\pi}}
\newcommand{\strat}{{\sigma}} %strategy
\newcommand{\cstrat}{\boldsymbol{\eta}}
\newcommand{\dstrat}{\boldsymbol{\delta}}
\newcommand{\feedback}{K}

\newcommand{\policySet}{{\Pi}}
\newcommand{\policySetCtrl}{{\Pi^\ctrl}}
\newcommand{\policySetDstb}{{\Pi^\dstb}}
\newcommand{\cstratSet}{\Gamma}
\newcommand{\dstratSet}{\Lambda}

\newcommand{\surfFunc}{{\psi}}
\newcommand{\distFunc}{s}
\newcommand{\consFunc}{{g}}
\newcommand{\consnxt}{{\consFunc'}}
\newcommand{\targFunc}{{\ell}}
\newcommand{\targnxt}{{\targFunc'}}
\newcommand{\mayerTerm}{{M}}
\newcommand{\lagrangian}{{L}}
\newcommand{\hamiltonian}{{H}}
\newcommand{\HJparticle}{{\Lambda}}

\newcommand{\target}{{\mathcal{T}}}
% \newcommand{\failure}{{\mathcal{F}}}
\newcommand{\constraint}{{\failure^\compl}}
% \newcommand{\constraint}{{\mathcal{K}}}
\newcommand{\safeSet}{{\Omega}}
\newcommand{\safeSetOpt}{{\safeSet^*}}
% \newcommand{\safeSetCBF}{{\safeSet^\cbf}}
\newcommand{\avoid}{{\mathcal{A}}}
\newcommand{\reach}{{\mathcal{R}}}
\newcommand{\reachErr}{{\hat{\reach}}}
% \newcommand{\reach}{{\hat\xSet}}
\newcommand{\reachBwd}{{\overleftarrow{\reach}}}
% \newcommand{\reachFwd}{{\overrightarrow{\reach}}}
\newcommand{\reachInev}{{\underline\reach}}
\newcommand{\reachRbst}{{\overline\reach}}
\newcommand{\reachOver}[2]{{\overline{\reach}^{#1}_{#2}}}
\newcommand{\reachavoid}{{\mathcal{RA}}}
\newcommand{\reachavoidInev}{{\underline\reachavoid}}
\newcommand{\reachavoidRbst}{{\overline\reachavoid}}
% \newcommand{\reachavoidBwd}{{\overleftarrow{\reachavoid}}}
% \newcommand{\reachavoidFwd}{{\overrightarrow{\reachavoid}}}
\newcommand{\tube}{{\mathcal{E}}}
\newcommand{\policyTrack}{{K_\tube}}
% \newcommand{\xCstrSet}{{\hat{\xSet}}}
% \newcommand{\cCstrSet}{{\hat{\cSet}}}


% CBF
% \newcommand{\cbfcstr}{{K^\text{CBF}}}
\newcommand{\cbf}{{h}}
\newcommand{\kFunc}{{\alpha}}


% Game Theory
\newcommand{\decision}{{\mathcal{D}}}
\newcommand{\utility}{{u}}

\newcommand{\iagent}{{i}}
\newcommand{\nagents}{{N}}
\newcommand{\indexSet}{{\mathcal{I}}}
\newcommand{\iagentaux}{{j}}

% \newcommand{\agent}{{\mathcal{A}}}
\newcommand{\agent}{{A}}
\newcommand{\agentCtrl}{{A^\ctrl}}
\newcommand{\agentDstb}{{A^\dstb}}
\newcommand{\ego}{{e}}
\newcommand{\query}{{q}}
\newcommand{\other}{{o}}


% Reinforcement Learning
\newcommand{\mdp}{{\mathcal{M}}}
\newcommand{\rl}{\mathop{\mathrm{RL}}}

\newcommand{\env}{{E}}
\newcommand{\envSpace}{{\mathcal{E}}}
\newcommand{\replay}{{\mathcal{D}}}

\newcommand{\return}{{G}}
\newcommand{\cost}{{c}}
\newcommand{\costTerm}{{m}}
\newcommand{\reward}{{r}}
\newcommand{\rewardTerm}{{m}}
\newcommand{\behDist}{{\rho}}
\newcommand{\policyBeh}{{\tilde{\policy}}}

\newcommand{\discount}{{\gamma}}
\newcommand{\reachavoidDiscount}{{\mathcal{RA}_\discount}}
\newcommand{\valDiscount}{{\valFunc_\discount}}
\newcommand{\qDiscount}{{\qFunc_\discount}}

\newcommand{\stateg}{{\mathbf{\state}}}
\newcommand{\ctrlg}{{\mathbf{\ctrl}}}
\newcommand{\xgSet}{{\mathbf{X}}}
\newcommand{\cgSet}{{\mathbf{U}}}
\newcommand{\trans}{{\mathbf{{{\bar{\dyn}}}}}}


% \newcommand{\stateSpace}{{\mathcal{S}}}
% \newcommand{\actionSpace}{{\mathcal{A}}}
% \newcommand{\costFuncSet}{{\mathcal{C}}}

\newcommand{\actorParam}{{\theta}}
\newcommand{\policyRnd}{{\policy^{\text{rnd}}}}
\newcommand{\policyRndAdv}{{\policy^{\text{rnd,+}}}}
\newcommand{\policyCtrl}{{\policy^\ctrl}}
\newcommand{\policyDstb}{{\policy^\dstb}}
\newcommand{\policyCtrlAux}{{\tilde{\policy}^\ctrl}}
\newcommand{\policyDstbAux}{{\tilde{\policy}^\dstb}}
\newcommand{\policyCtrlOpt}{{\policy^{\ctrl*}}}  % {{\policy^{\ctrl*}}}
% \newcommand{\policyDstbOpt}{{\policy^{\dstb*}}}
\newcommand{\policyDstbOpt}{{\actorDstb^*}}
% \newcommand{\actorParamCtrl}{{\actorParam^\ctrl}}
% \newcommand{\actorParamDstb}{{\actorParam^\dstb}}
\newcommand{\actorParamCtrl}{{\theta}}
\newcommand{\actorParamDstb}{{\psi}}
\newcommand{\criticParam}{{\omega}}
\newcommand{\criticauxParam}{{\omega'}}
\newcommand{\criticVal}{{\valFunc_{\criticParam}}}
\newcommand{\critic}{{\qFunc_{\criticParam}}}
\newcommand{\criticaux}{{\qFunc_\criticauxParam}}
\newcommand{\actor}{{\policy_\actorParam}}
\newcommand{\actorCtrl}{{\policy_\actorParamCtrl}}
\newcommand{\actorDstb}{{\policy_\actorParamDstb}}
% \newcommand{\policyISAACS}{{\policy^\text{ISAACS}}}
\newcommand{\policyISAACS}{{\actorCtrl}}

\newcommand{\lr}{{\lambda}}
\newcommand{\lrterm}{{\lr_{\min}}}
\newcommand{\lrActor}{{\lr_{\actorParam}}}
\newcommand{\lrCtrl}{{\lr_{\actorParamCtrl}}}
\newcommand{\lrDstb}{{\lr_{\actorParamDstb}}}
\newcommand{\lrCritic}{{\lr_{\criticParam}}}
\newcommand{\lrEnt}{{\lr_{\entCoeff}}}
% \newcommand{\lrTarget}{{\lr_{\criticauxParam}}}
\newcommand{\lrTarget}{{\tau}}
\newcommand{\updateRatio}{{\rho}}

\newcommand{\entCoeff}{{\alpha}}
\newcommand{\entCoeffCtrl}{{\entCoeff^\ctrl}}
\newcommand{\entCoeffDstb}{{\entCoeff^\dstb}}
\newcommand{\entTarget}{{\entropy_{\min}}}

\newcommand{\done}{{\phi}}
% }


% Shielding
% \newcommand{\shield}{{\text{sf}}}
\newcommand{\shield}{\text{\tiny{\faShield*}}}
\newcommand{\shieldset}{\mathcal{S}}
\newcommand{\task}{{\text{task}}}
\newcommand{\safety}{{\text{s}}}
\newcommand{\nncs}[2]{{{#1}_{#2}}}
\newcommand{\monitor}{{\Delta}^\shield}
% \newcommand{\monitor}{{\Delta}}
\newcommand{\monitorSet}{{\boldsymbol{\Delta}}}
\newcommand{\policyTask}{{\policy^\task}}
% \newcommand{\policyExec}{{\policy^\text{exec}}}
\newcommand{\policyExec}{{\safetyFilter^\text{prev}}}
\newcommand{\fallback}{{\policy^\shield}}
\newcommand{\fallbackOpt}{{\policy^{\shield*}}}
\newcommand{\intervention}{{\iota^\shield}}
\newcommand{\safetyFilter}{{\phi}}
\newcommand{\safetyFilterValue}{{\safetyFilter^{\text{critic}}}}
\newcommand{\safetyFilterRoll}{{\safetyFilter^{\text{game}}}}
% \newcommand{\safetyFilterCBF}{{\phi^\text{CBF}}}
\newcommand{\modulator}{{\mathcal{I}}}
\newcommand{\policyInv}[1]{{\policy^{#1}}}
% \newcommand{\monitorCBF}{\Delta^\cbf}
\newcommand{\monitorCritic}{\Delta^{\shield,\text{critic}}_{\epsilon}}
\newcommand{\monitorAvoidNom}{\Delta^{\shield,\text{nom}}_{\khorizon,\avoid}}
\newcommand{\monitorRANom}{\Delta^{\shield,\text{nom}}_{\khorizon,\reachavoid}}
\newcommand{\monitorAvoidFRS}{\Delta^{\shield,\text{FRS}}_{\khorizon,\avoid}}
\newcommand{\monitorRAFRS}{\Delta^{\shield,\text{FRS}}_{\khorizon,\reachavoid}}
\newcommand{\monitorAvoidGame}{\Delta^{\shield,\text{game}}_{\khorizon,\phorizon,\avoid}}
\newcommand{\monitorRAGame}{\Delta^{\shield,\text{game}}_{\khorizon,\phorizon,\reachavoid}}
\newcommand{\monitorRAGameNo}{\Delta^{\shield,\text{game}}_{\khorizon,\reachavoid}}
\newcommand{\monitorGame}{\Delta^{\shield,\text{game}}_{}}

% Imitation Learning
\newcommand{\featureMap}{\phi}
\newcommand{\rewardParam}{{w}}
\newcommand{\rewardParamOpt}{{w^*}}
\newcommand{\rewardParamSet}{\mathcal{W}}

% \newcommand{\trajDemo}{\Xi_D}
\newcommand{\trajDemo}{{\mathcal{D}}}
\newcommand{\ddata}{{\mathcal{D}}}
\newcommand{\qdata}{\mathbf{\boldsymbol \query}}
% \newcommand{\fdata}{\mathbf{\boldsymbol \feedback}}
\newcommand{\rdata}{\mathbf{\boldsymbol \rewardFunc}}

\newcommand{\irl}{\mathop{\mathrm{IRL}}}
\newcommand{\confCoeff}{\beta}
% \newcommand{\constraintSubset}{{\mathcal{K}}}

\newcommand{\design}{d}
\newcommand{\feature}{f}
\newcommand{\designSpace}{D}
% \newcommand{\feedback}{\zeta}


%== Multi-Objective Optimization ==
\newcommand{\obj}{f}


% == NVIDIA ==
\newcommand{\map}{{m}}
\newcommand{\resp}{{\beta}}
\newcommand{\horizonFut}{{T_f}}
\newcommand{\horizonHis}{{T_h}}
\newcommand{\csigPredSet}[2]{{\csigSet_{#2}^{#1}}}
% \newcommand{\csigPred}[1]{{\hat{\csig}^{#1}}}
\newcommand{\csigPred}[1]{{\csig}^{#1}}
\newcommand{\csigHis}[2]{{\csig^{#1}_{#2-\horizonHis:#2}}}
\newcommand{\trajPredSet}[2]{{\trajSet_{#2}^{#1}}}
\newcommand{\trajPred}[1]{{\hat{\traj}^{#1}}}
\newcommand{\trajHis}[2]{{\traj^{#1}_{#2-\horizonHis:#2}}}
\newcommand{\cvaeInput}{{\mathbf{x}}}
\newcommand{\cvaeOutput}{{\mathbf{y}}}
\newcommand{\latent}{{z}}
\newcommand{\nlevels}{{H}}

% Measurement units
\newcommand{\s}{~\text{s}}
\newcommand{\m}{~\text{m}}
\newcommand{\ms}{~\text{m}/\text{s}}
\newcommand{\mss}{~\text{m}/\text{s}^2}
\providecommand{\rad}{~\text{rad}}
\newcommand{\rads}{~\text{rad}/\text{s}}
\newcommand{\kg}{~\text{kg}}
\newcommand{\Npm}{~\text{N}/\text{m}}
\newcommand{\newton}{~\text{N}}
\newcommand{\Nm}{~\text{Nm}}
\newcommand{\Hz}{~\text{Hz}}

% Robot
% \newcommand{\yaw}{{\ang_{\text{y}}}}
% \newcommand{\pitch}{{\ang_{\text{p}}}}
% \newcommand{\roll}{{\ang_{\text{r}}}}
\newcommand{\yaw}{{\ang_{z}}}
\newcommand{\pitch}{{\ang_{y}}}
\newcommand{\roll}{{\ang_{x}}}
\newcommand{\yawdot}{{\angvel_z}}
\newcommand{\pitchdot}{{\angvel_y}}
\newcommand{\rolldot}{{\angvel_x}}
\newcommand{\steer}{{\delta}}
\newcommand{\steerdot}{{\angvel}}
\newcommand{\wheelbase}{{L}}

\newcommand{\pos}{{p}}
\newcommand{\posx}{{\pos_x}}
\newcommand{\posy}{{\pos_y}}
\newcommand{\posz}{{\pos_z}}
\newcommand{\vel}{{v}}
\newcommand{\velx}{{\vel_x}}
\newcommand{\vely}{{\vel_y}}
\newcommand{\velz}{{\vel_z}}
\newcommand{\accel}{{a}}

\newcommand{\force}{{F}}
\newcommand{\forcex}{{\force_x}}
\newcommand{\forcey}{{\force_y}}
\newcommand{\forcez}{{\force_z}}
\newcommand{\forceposx}{{\pos^\force_x}}
\newcommand{\forceposy}{{\pos^\force_y}}
\newcommand{\forceposz}{{\pos^\force_z}}

\newcommand{\bound}{{\text{b}}}
\newcommand{\obst}{{\text{o}}}



==> sections/related.tex <==
\section{Related Work}
\label{sec:related}

\textbf{Learning for Locomotion.}
Conventionally, legged locomotion has been addressed through model-based techniques, including model-predictive control~\citep{bledt2018mit} and trajectory optimization~\citep{winkler2018gait}.
However, recent advancements in deep learning offer the opportunity to learn directly from interactions with environments and feedback in the form of a reward signal, bypassing the need for intricate dynamics modeling and extensive domain knowledge. %~\citep{zhuang2023robot}
%
\citet{kostrikov2023demonstrating} demonstrated the direct training of locomotion policies across various terrains in the real world through reinforcement learning by carefully formulating the problem with consideration for state space, action space, and reward function.
Despite the success of reinforcement learning, it relies on trial and error during training. In safety-critical environments, learning from scratch can lead to catastrophic safety failures.
An alternative approach involves initially training control policies in simulation and then bridging the simulation-to-real gap through methods such as domain randomization~\citep{tobin2017domain}, task-driven adaptation~\citep{kumar2021rma, ren2023adaptsim}, and system identification~\citep{fabio2019bayessim}.

\textbf{Safety Filters.}
While learning-based policies discussed earlier exhibit practical utility, they primarily focus on task-oriented performance metrics.
However, ensuring their safe operation in unforeseen, uncertain, and unforgiving environments is of paramount importance. 
A recent line of work aims at inducing safety awareness and even guarantees for learning-based policies through a \emph{safety filter}.
The runtime operation of every safety filter can be conceptualized as two interrelated functions: \emph{monitoring} and \emph{intervention}~\citep{hsu2023safety}.
The safety filter continually monitors the robot's planned actions to assess the level of safety risk.
Subsequently, the filter may intervene by modulating or entirely overriding the robot's intended control input to guarantee the preservation of safety.
Many safety filters incorporate monitoring and intervention procedures guided by a safety-oriented control strategy, which the filter views as a viable \emph{fallback}.

One important family of safety filters is built on Hamilton-Jacobi (HJ) reachability analysis, which computes a global safe value function through dynamic programming~\citep{mitchell2008flexible,fisac2015reachavoid}.
The resulting value function encodes the maximal safe set and optimal safety \remove{policy }\new{fallback}, and thus, a \emph{least-restrictive} safety filter can be synthesized by a \emph{switch-type} intervention~\citep{fisac2019AGS}.
Although systematic and powerful, HJ methods have poor scalability and are limited to no more than 6 state dimensions~\citep{bui2022optimizeddp}.

On the other hand, control barrier functions (CBFs)~\citep{ames2017cbf,ames2019control} no longer encode or approximate the maximal safe set. Instead, CBFs, if found, provide a sufficient condition to keep the system safe forever, akin to control Lyapunov functions~\citep{sontag1983lyapunov}.
Another critical feature of CBFs is their usage of \emph{optimization-type} intervention, which finds minimal modulation to the task-oriented control that still keeps the system safe, and thus CBFs allow a smooth intervention mechanism.
However, finding a CBF for general dynamics is usually not trivial, and CBF is only local and not robust to model mismatch.

For high-dimensional dynamics, computing global optimal value functions (HJ) is computationally prohibitive, and finding a valid CBF is often heuristic.
Instead of relying on value functions, model predictive safety filters aim to certify the system safety in real time by forward simulating (``rolling out'') or trajectory optimization,\footnote{Some recent efforts have been made to synthesize CBFs based on model predictive methods~\citep{chen2021backup,kumar2023cbfddp}, while the concerned dynamics has no more than 5 state dimensions.}~\citep{wabersich2018linear,bastani2021safe,hsunguyen2023isaacs} which closely link to this work.
\citet{hsunguyen2023isaacs} consider the forward-reachable set (FRS) of the system trajectories. However, the use of FRS brings two challenges for general high-dimensional dynamics: 1) FRS needs to be tight to make safety filters not overly conservative, and 2) the computation of FRS needs to be quick to satisfy real-time constraints.
Instead, \citet{bastani2021safe} assume disturbance distribution is known, by which a sufficient number of trajectories are sampled and a statistical guarantee is derived; nonetheless, disturbance distribution may be difficult to obtain in practice.
% Model predictive safety filters, on the other hand, monitor the system safety through solving a trajectory optimization problem~\citep{kousik2020bridging,wabersich2022probabilistic} or by forward simulating (``rolling out'') the dynamics model with accumulating uncertainty~\citep{hsunguyen2023isaacs,bastani2021safe}, which closely link to this work.

Safety filters have been applied to ensure the safe operation of learning-based locomotion~\citep{hsuzen2022sim2lab2real,yang2022safe}.
\citet{hsuzen2022sim2lab2real} introduce a safety monitor based on a value function and fine-tune the corresponding safety filter using a two-stage reinforcement learning framework, providing statistical safety guarantees.
However, they consider the uncertainty distribution as a whole, while our work focuses on robustly safeguarding against the worst-case realization of uncertainty. 
\citet{yang2022safe} propose a safety monitor criterion based on a heuristically defined safety-triggered set, checking if rollouts activate the criterion.
In contrast, our work determines such a safety-triggered set through gameplay rollouts.
Additionally, these methods employ a simplified dynamics model and only consider velocity control instead of torque or joint position control directly.
